Text-Conditional Contextualized Avatars For Zero-Shot Personalization

Recent large-scale text-to-image generation models have made significant improvements in the quality, realism, and diversity of the synthesized images and enable users to control the created content through language. However, the personalization aspect of these generative models is still challenging and under-explored. In this work, we propose a pipeline that enables personalization of image generation with avatars capturing a user's identity in a delightful way. Our pipeline is zero-shot, avatar texture and style agnostic, and does not require training on the avatar at all - it is scalable to millions of users who can generate a scene with their avatar. To render the avatar in a pose faithful to the given text prompt, we propose a novel text-to-3D pose diffusion model trained on a curated large-scale dataset of in-the-wild human poses improving the performance of the SOTA text-to-motion models significantly. We show, for the first time, how to leverage large-scale image datasets to learn human 3D pose parameters and overcome the limitations of motion capture datasets.

==> avatar-personalization (6)/Tables/ablation_table.tex <==
\begin{table}[t]
    \begin{center}
        \setlength{\tabcolsep}{2pt}
            \begin{tabular}{lccc}
                \toprule
                \textbf{Method} & 
                Training data &
                Human Eval $\uparrow$ &
                CLIPSIM  $\uparrow$ \\
                \midrule
                6D+VPoser  &
                HumanML3D &
                69.8 &
                0.149 \\
                6D  &
                ITPP &
                56.6 &
                0.146 \\
                VPoser &
                ITPP &
                51.5 &
                0.150 \\
                6D+VPoser &
                ITPP &
                - &
                0.149 \\

                \bottomrule
            \end{tabular}
    \caption{\textbf{Ablation study of different pose representations and training datasets}: HumanML3D dataset was modified for single frame pose generation. The human evaluation text faithfulness is reported as the percentage of the majority vote raters that preferred the last line setting over the others on our curated 390 prompts set, i.e., any value above 50\% means 6D+Vposer trained on our ITPP data was favored. For CLIP similarity, we rendered SMPL avatars using the 3D pose predicted by our model. }
    \vspace{-2em}
    \label{tab:ablation_data}
    \end{center}
\end{table}


==> avatar-personalization (6)/Tables/image_generation_human_eval.tex <==
\begin{table}[t]
    \begin{center}
        \setlength{\tabcolsep}{2pt}
            \begin{tabular}{lccc}
                \toprule
                \textbf{Method} & 
                Avatar $\uparrow$ & 
                Text $\uparrow$ &
                CLIPSIM  $\uparrow$
                \\
                &
                match & 
                match &
                \\
                \midrule
                 Baseline &
                - &
                - &
                0.239
                \\

                Fine-tuned &
                0.56 &
                0.48 &
                0.239
                \\

                Ours  &
                \textbf{0.63} &
                \textbf{0.52} &
                \textbf{0.242}
                \\

                \bottomrule
            \end{tabular}
    \caption{\textbf{Personalized Image Generation Evaluation:} We evaluated our method against an inpainting/outpainting baseline. We report human evaluation (avatar and text faithfulness) and automatic metrics (CLIP similarity). The results for the human evaluation are reported as the percentage of the majority vote raters that preferred our method over the baseline, i.e., any value above 50\% means our method was favored. The ``fine-tuned'' method is the inpainting/outpainting model fine-tuned on our ITPP dataset, and isolates the value of the architecture modifications we made.}
    \vspace{-2em}
    \label{tab:image_gen_eval}
    \end{center}
\end{table}

==> avatar-personalization (6)/Tables/pose_generation_auto_eval.tex <==
\begin{table}[t]
    \begin{center}
        \setlength{\tabcolsep}{2pt}
            \begin{tabular}{lccc}
                \toprule
                \textbf{Method} & 
                Human Eval $\uparrow$ &
                FPD $\downarrow$ & 
                CLIPSIM $\uparrow$ \\
                \midrule
                TEMOS \cite{petrovich2022temos} &
                73.7 &
                4.6 &
                0.17 \\
                MotionCLIP \cite{tevet2022motionclip} &
                59.0 &
                12.06 &
                0.145 \\
                AvatarCLIP \cite{hong2022avatarclip}  &
                60.7 &
                13.28 &
                0.162 \\
                MDM \cite{tevet2022mdm}  &
                60.0 &
                11.16 &
                0.15 \\
                 \bottomrule
                PAS (6D+VPoser) &
                - &
                6.25 &
                0.16 \\
                PAS (VPoser) &
                - &
                7.27 &
                0.164 \\
                \bottomrule
            \end{tabular}
    \caption{\textbf{Text-to-3D Pose Generation Evaluation:} We evaluate our method, PAS, against text-to-motion generation baselines. We report human evaluation scores where we compare each baseline against our model in terms of the correctness of each generated pose given a text prompt. The results are reported as the percentage of the majority vote raters that preferred our method to each baseline on our curated 390 prompts set. FPD measures overall quality and diversity of the samples, and CLIPSIM measures pose-text faithfulness; Both evaluated on the HumanML3D test set. Our model is trained on our ITPP dataset and HumanML3D train set.}
    \vspace{-2em}
    \label{tab:pose_gen_eval}
    \end{center}
\end{table}
